On the Complexity of Sub-Tree Scheduling for Wireless Sensor Networks with Partial Coverage

Given an undirected graph $G$ whose edge weights change over $s$ time slots, the sub-tree scheduling for wireless sensor networks with partial coverage asks to partition the vertices of $G$ in $s$ non-empty trees such that the total weight of the trees is minimized. In this note we show that the problem is NP-hard in both the cases where $s$ $(i)$ is part of the input and $(ii)$ is a fixed instance parameter. In both our proofs we reduce from the cardinality Steiner tree problem. We additionally give polynomial-time algorithms for structured inputs of the problem.

==> fig1.tex <==
\begin{figure}%[ht]
\centering

\subfigure[][]{
\resizebox{0.24\textwidth}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[rectangle,scale=1.2] (t3) at (12,0) {3};
\node[rectangle,scale=1.2] (t5) at (6,3.5) {5};
\node[rectangle,scale=1.2] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);
%\draw [dashed] (S2) -- (5);

\end{tikzpicture}
}
}
\subfigure[][]{
\resizebox{0.47\textwidth}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[diamond,scale=0.6] (t301) at (14,1.5) {\Large $v^3_1$};
\node[diamond,scale=0.6] (t302) at (14,0) {\Large $v^3_2$};
\node[diamond,scale=0.6] (t303) at (14,-1.5) {\Large $v^3_3$};


\node[rectangle,scale=1] (t3) at (12,0) {3};

\node[diamond,scale=0.6] (t501) at (4,5) {\Large $v^5_1$};
\node[diamond,scale=0.6] (t502) at (4,3.5) {\Large $v^5_2$};
\node[diamond,scale=0.6] (t503) at (4,2) {\Large $v^5_3$};


\node[rectangle,scale=1] (t5) at (6,3.5) {5};

\node[diamond,scale=0.6] (t601) at (16,5) {\Large $v^6_1$};
\node[diamond,scale=0.6] (t602) at (16,3.5) {\Large $v^6_2$};
\node[diamond,scale=0.6] (t603) at (16,2) {\Large $v^6_3$};


\node[rectangle,scale=1] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);

\draw [dashed] (t601) -- (t6);
\draw [dashed] (t602) -- (t6);
\draw [dashed] (t603) -- (t6);

\draw [dashed] (t501) -- (t5);
\draw [dashed] (t502) -- (t5);
\draw [dashed] (t503) -- (t5);

\draw [dashed] (t301) -- (t3);
\draw [dashed] (t302) -- (t3);
\draw [dashed] (t303) -- (t3);

\end{tikzpicture}
}
}
\caption{Example of a CST instance (a),  in which terminal vertices are squared-shaped, and of the corresponding \pb{} instance for $k = 4$ (b), in which fictitious vertices are diamond-shaped.}\label{fig:non-fixed}
\end{figure}


==> fig2-BIS.tex <==
\begin{figure}%[ht]
\centering

\subfigure[][]{
\resizebox{0.25\textwidth}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[rectangle,scale=1.2] (t3) at (12,0) {3};
\node[rectangle,scale=1.2] (t5) at (6,3.5) {5};
\node[rectangle,scale=1.2] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);
%\draw [dashed] (S2) -- (5);

\end{tikzpicture}
}
}
\subfigure[][]{
\resizebox{0.4\textwidth}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[diamond,scale=0.6] (t301) at (14,0.75) {\Large $v^3_1$};
\node[diamond,scale=0.6] (t302) at (14,-0.75) {\Large $v^3_2$};


\node[rectangle,scale=1] (t3) at (12,0) {3};

\node[diamond,scale=0.6] (t501) at (4,4.25) {\Large $v^5_1$};
\node[diamond,scale=0.6] (t502) at (4,2.75) {\Large $v^5_2$};


\node[rectangle,scale=1] (t5) at (6,3.5) {5};

\node[diamond,scale=0.6] (t601) at (14,4.25) {\Large $v^6_1$};
\node[diamond,scale=0.6] (t602) at (14,2.75) {\Large $v^6_2$};

\node[rectangle,scale=1] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);

\draw [dashed] (t601) -- (t6);
\draw [dashed] (t602) -- (t6);

\draw [dashed] (t501) -- (t5);
\draw [dashed] (t502) -- (t5);

\draw [dashed] (t301) -- (t3);
\draw [dashed] (t302) -- (t3);

\draw [densely dotted] (2) -- (4);
\draw [densely dotted] (2) -- (t5);
\draw [densely dotted] (2) -- (t6);
\draw [densely dotted] (2) .. controls(7.5,2) .. (7);

\draw [densely dotted] (t3) .. controls(9,0.5) .. (t5);
\draw [densely dotted] (t3) -- (t6);
\draw [densely dotted] (t3) -- (7);

\draw [densely dotted] (4) -- (7);

\draw [densely dotted] (t5) -- (t6);

\draw [densely dotted] (t6) .. controls(9,0.5) .. (1);


\end{tikzpicture}
}
}
\caption{Example of a CST instance (a), in which terminal vertices are squared-shaped, and of the corresponding \pb{} instance for $\bar s = 3$ (b), in which fictitious vertices are diamond-shaped.}\label{fig:fixed}
\end{figure}


==> fig2.tex <==
\begin{figure}%[ht]
\centering

\subfigure[][]{
\resizebox{5.8cm}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[rectangle,scale=1.2] (t3) at (12,0) {3};
\node[rectangle,scale=1.2] (t5) at (6,3.5) {5};
\node[rectangle,scale=1.2] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);
%\draw [dashed] (S2) -- (5);

\end{tikzpicture}
}
}
\subfigure[][]{
\resizebox{9.8cm}{!}{
\begin{tikzpicture}[scale=.45, transform shape]
\tikzstyle{every node} = [circle,scale=1.5,fill=white,draw=black]

\node[diamond,scale=0.6] (t30) at (14,0) {$v^3$};

\node[rectangle,scale=1] (t3) at (12,0) {3};

\node[diamond,scale=0.6] (t50) at (4,3.5) {$v^5$};

\node[rectangle,scale=1] (t5) at (6,3.5) {5};

\node[diamond,scale=0.6] (t60) at (14,3.5) {$v^6$};

\node[rectangle,scale=1] (t6) at (12,3.5) {6};

\node (1) at (6,0.0) {1};
\node (2) at (9.0,-2.0) {2};
\node (4) at (9,1.75) {4};
\node (7) at (9,5.0) {7};

\draw (1) -- (2);
\draw (1) -- (t5);
\draw (1) -- (4);
\draw (t3) -- (1);
\draw (t3) -- (2);
\draw (t3) -- (4);
\draw (4) -- (t5);
\draw (4) -- (t6);
\draw (t5) -- (7);
\draw (t6) -- (7);

\draw [dashed] (t60) -- (t6);

\draw [dashed] (t50) -- (t5);

\draw [dashed] (t30) -- (t3);

\draw [densely dotted] (2) -- (4);
\draw [densely dotted] (2) -- (t5);
\draw [densely dotted] (2) -- (t6);
\draw [densely dotted] (2) .. controls(7.5,2) .. (7);

\draw [densely dotted] (t3) .. controls(9,0.5) .. (t5);
\draw [densely dotted] (t3) -- (t6);
\draw [densely dotted] (t3) -- (7);

\draw [densely dotted] (4) -- (7);

\draw [densely dotted] (t5) -- (t6);

\draw [densely dotted] (t6) .. controls(9,0.5) .. (1);

\end{tikzpicture}
}
}
\caption{Example of a CST instance (a) and of the corresponding \pb{} instance for $\bar s = 2$ (b)}\label{fig:fixed}
\end{figure}

